Utilizing Adversarial Examples for Bias Mitigation and Accuracy Enhancement

We propose a novel approach to mitigate biases in computer vision models by utilizing counterfactual generation and fine-tuning. While counterfactuals have been used to analyze and address biases in DNN models, the counterfactuals themselves are often generated from biased generative models, which can introduce additional biases or spurious correlations. To address this issue, we propose using adversarial images, that is images that deceive a deep neural network but not humans, as counterfactuals for fair model training. Our approach leverages a curriculum learning framework combined with a fine-grained adversarial loss to fine-tune the model using adversarial examples. By incorporating adversarial images into the training data, we aim to prevent biases from propagating through the pipeline. We validate our approach through both qualitative and quantitative assessments, demonstrating improved bias mitigation and accuracy compared to existing methods. Qualitatively, our results indicate that post-training, the decisions made by the model are less dependent on the sensitive attribute and our model better disentangles the relationship between sensitive attributes and classification variables.

==> sec/5_experiment_setup.tex <==
\section {Experiment Setup}
\label{sec:exp_setup}
This section describes our experimental setup. We outline the datasets used, followed by the evaluation metrics that are employed to evaluate the model and finally describe the training details.

\subsection{Datasets}
\label{sub:dataset}
Similar to Wang et al.'s approach \cite{wang2022assessing}, we use the CelebA \cite{liu2015faceattributes} and LFW \cite{LFWTech} datasets. CelebA contains 202,599 images annotated with 40 attributes and we focus on Smiling, Big Nose, and Wavy Hair, with Gender as the protected attribute. Similarly, LFW comprises 13,244 images annotated with 73 attributes, where we select Smile, Wavy Hair, and Bags Under Eyes, with Gender as the protected attribute.

%Similar to the methodology employed by Wang et al.\cite{wang2022assessing}, we have chosen the CelebA\cite{liu2015faceattributes} and LFW \cite{LFWTech} datasets for our experiments. The CelebA dataset \cite{liu2015faceattributes} contains 202,599 images, each annotated with 40 distinct attributes. In our analysis, we focus on three target attributes: Smiling, Big Nose, and Wavy Hair, with Gender serving as the protected attribute. Similarly, in the LFW dataset \cite{LFWTech}, which consists of 13,244 images, each labeled with 73 attributes, we select Smile, Wavy Hair, and Bags Under Eyes, once more with Gender as the protected attribute.

%As an alternative experiment we also train a  Pleural Effusion  classification using the Chexpert dataset \cite{irvin2019chexpert}, which consists of chest radiographs. The Chexpert dataset comprises 223,648 images from 64,740 patients, with labels indicating the presence of 14 common chest radiograph observations. Additionally, the dataset provides information on the patients' sex and age. Radiograph observations are classified as positive, negative, or with an uncertainty value, which we will use for training purposes. Similar to the CelebA dataset sex is taken as the protected attribute in the dataset.

\subsection{Evaluation Metrics}
\label{sub:eval_metrics}
To evaluate the fairness of our model, we employ three key metrics: the Difference in Demographic Parity (DDP), the Difference in Equalized Odds (DEO), and the Difference in Equalized Opportunity (DEOp) \cite{hardt2016equality}. Alongside these, we also measure the model's accuracy (ACC). Lower values for fairness metrics indicate a less biased model whereas a high value in accuracy indicates a more performant model. For more details about the metrics and their definition please refer to the supplementary material (Sections \ref{sup: Deifintion} and \ref{sup:metrics}).

%DDP quantifies the absolute gap in approval rates across different classes in the protected attribute. A heightened DDP value suggests a tendency for individuals in the more advantaged group to receive more favorable outcomes than their counterparts in the less advantaged group. Ideally, this value should be zero, indicating no disparity. Conversely, DEO focuses on the difference in the rates of false negatives and false positives between the classes of the protected attribute. A substantial DEO indicates a bias in which the more advantaged group is either less likely to be incorrectly dismissed or more likely to be inaccurately favored. The goal here is to minimize the DEO, striving for more equitable error rates across different groups. Lastly, DEOp measures the disparity in True Positive Rates between different demographic groups in a model, indicating bias in favorable outcomes. A DEOp of zero indicates equal accuracy across groups, representing a fairness ideal in model performance.

\subsection{Training Details}
\label{sub:train_details}
We utilize ResNet-18 \cite{he2016deep} as the backbone architecture, pretrained for 50 epochs and fine-tuned with our proposed approach for 10 epochs, utilizing the same data distribution $D$. A batch size of 128 is used with Adam optimizer (learning rate $10^{-4}$). We experiment with $\epsilon \in [0,1]$ for varying adversarial noise levels in images, with smaller $\epsilon$ implying less noise and values closer to 1 indicating higher corruption.

%For all models trained/fine-tuned, we use ResNet-$18$ \dhruv{missing citation}\cite{he2016deep} as the backbone architecture. The models are pre-trained for $50$ epochs and fine-tuned using the method for adversarial counter tuning for $15$ epochs. We use a batch size of $128$ and train the model using the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$. We experiment with different values of $\epsilon \in [0,1]$ \lee{what are the exact values?} to inject varying amounts of adversarial noise in the images. A smaller value of $\epsilon$ signifies less adversarial noise added to images while values closer to $1$ indicate that the images have been largely corrupted.
